M2: Mixed Models with Preferences, Popularities and Transitions for Next-Basket Recommendation

Next-basket recommendation considers the problem of recommending a set of items into the next basket that users will purchase as a whole. In this paper, we develop a novel mixed model with preferences, popularities and transitions (M2) for the next-basket recommendation. This method models three important factors in next-basket generation process: 1) users' general preferences, 2) items' global popularities and 3) transition patterns among items. Unlike existing recurrent neural network-based approaches, M2 does not use the complicated networks to model the transitions among items, or generate embeddings for users. Instead, it has a simple encoder-decoder based approach (ed-Trans) to better model the transition patterns among items. We compared M2 with different combinations of the factors with 5 state-of-the-art next-basket recommendation methods on 4 public benchmark datasets in recommending the first, second and third next basket. Our experimental results demonstrate that M2 significantly outperforms the state-of-the-art methods on all the datasets in all the tasks, with an improvement of up to 22.1%. In addition, our ablation study demonstrates that the ed-Trans is more effective than recurrent neural networks in terms of the recommendation performance. We also have a thorough discussion on various experimental protocols and evaluation metrics for next-basket recommendation evaluation.

==> ablationThree.tex <==
\begin{table}[!h]
  \caption{Ablation Study on Recommending Third Next Basket}
  \label{tbl:ablationOne}
  \centering
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{1pt}}l@{\hspace{1pt}}
	@{\hspace{1pt}}l@{\hspace{1pt}}          
	@{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
	}
        \toprule
        dataset & factors & recall@5 & recall@10 & recall@20 & ndcg@5 & ndcg@10 & ndcg@20\\
        \midrule
        \multirow{5}{*}{TaFeng}
        & \GP & 0.1037 & 0.1415 & 0.1907 & 0.1114 & 0.1207 & 0.1360\\ 
        & \IT & 0.0557 & 0.0728 & 0.1003 & 0.0621 & 0.0649 & 0.0736\\
        & $\GP$+$\IT$ & 0.1179 & 0.1620 & 0.2121 & 0.1229 & 0.1341 & 0.1501\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.1186 & 0.1540 & 0.2046 & 0.1207 & 0.1291 & 0.1451\\
        %\cmidrule(l){2-6}
        %& imprv     & 3.8\% & 1.2\% & 7.6\% & 14.2\% \\
        \midrule
        \multirow{5}{*}{TMall}
        & \GP & 0.1522 & 0.1925 & 0.2308 & 0.1096 & 0.1209 & 0.1306\\
        & \IT & 0.1130 & 0.1225 & 0.1313 & 0.0902 & 0.0928 & .0951\\
        & $\GP$+$\IT$ & 0.1542 & 0.1966 & 0.2380 & 0.1139 & 0.1264 & 0.1365\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.1575 & 0.1999 & 0.2394 & 0.1151 & 0.1271 & 0.1370\\
        \midrule
        \multirow{5}{*}{sTMall}
        & \GP & 0.1267 & 0.1610 & 0.1872 & 0.0984 & 0.1087 & 0.1155\\
        & \IT & 0.1012 & 0.1073 & 0.1134 & 0.0893 & 0.0912 & 0.0928\\
        & $\GP$+$\IT$ & 0.1367 & 0.1698 & 0.1961 & 0.1086 & 0.1188 & 0.1256\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.1364 & 0.1723 & 0.1982 & 0.1087 & 0.1198 & 0.1266\\
        \midrule
        \multirow{5}{*}{Gowalla}
        & \GP & 0.5092 & 0.5751 & 0.6251 & 0.4282 & 0.4509 & 0.4649\\
        & \IT & 0.0183 & 0.0300 & 0.0445 & 0.0124 & 0.0167 & 0.0208\\
        & $\GP$+$\IT$ & 0.4774 & 0.5453 & 0.5963 & 0.3929 & 0.4163 & 0.4304\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.5147 & 0.5804 & 0.6316 & 0.4307 & 0.4532 & 0.4674\\
        %\cmidrule(l){2-6}
        %& imprv     & 0.1\% & 0.2\% & -0.1\% & 0.1\% \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
        \begin{footnotesize}
        \item
        \method is identical to $\GP$+$\IT$+$\IC$. 
          The best performance in each dataset is \textbf{bold}.
          The second best performance is \underline{underline}.
          %\xia{modify this table as we discussed... for sTMall under recall@10, bold 0.1226 for EMLR and underline 
          %the two 0.1226 for MLP+GP and RNN+GP, and calculate improve accordingly... }
          \par
        \end{footnotesize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> ablationTwo.tex <==
\begin{table}[!h]
  \caption{Ablation Study on Recommending Second Next Basket}
  \label{tbl:ablationOne}
  \centering
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{1pt}}l@{\hspace{1pt}}
	@{\hspace{1pt}}l@{\hspace{1pt}}          
	@{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
        @{\hspace{1pt}}r@{\hspace{1pt}}
	}
        \toprule
        dataset & factors & recall@5 & recall@10 & recall@20 & ndcg@5 & ndcg@10 & ndcg@20\\
        \midrule
        \multirow{5}{*}{TaFeng}
        & \GP & 0.0920 & 0.1313 & 0.1787 & 0.1056 & 0.1138 & 0.1293\\ 
        & \IT & 0.0571 & 0.0775 & 0.1011 & 0.0620 & 0.0665 & 0.0744\\
        & $\GP$+$\IT$ & 0.1097 & 0.1524 & 0.2095 & 0.1199 & 0.1290 & 0.1480\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.1106 & 0.1529 & 0.2086 & 0.1204 & 0.1293 & 0.1477\\
        %\cmidrule(l){2-6}
        %& imprv     & 3.8\% & 1.2\% & 7.6\% & 14.2\% \\
        \midrule
        \multirow{5}{*}{TMall}
        & \GP & 0.1253 & 0.1556 & 0.1904 & 0.0959 & 0.1052 & 0.1144\\
        & \IT &  0.1126 & 0.1207 & 0.1305 & 0.0995 & 0.1018 & 0.1046\\
        & $\GP$+$\IT$ & 0.1394 & 0.1697 & 0.2016 & 0.1065 & 0.1159 & 0.1244\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.1402 & 0.1711 & 0.2008 & 0.1070 & 0.1168 & 0.1248\\
        \midrule
        \multirow{5}{*}{sTMall}
        & \GP & 0.1132 & 0.1398 & 0.1563 & 0.0885 & 0.0968 & 0.1011\\
        & \IT & 0.0990 & 0.1056 & 0.1113 & 0.0892 & 0.0912 & 0.0926\\
        & $\GP$+$\IT$ & 0.1260 & 0.1528 & 0.1717 & 0.1025 & 0.1110 & 0.1160\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.1259 & 0.1530 & 0.1723 & 0.1031 & 0.1116 & 0.1167\\
        \midrule
        \multirow{5}{*}{Gowalla}
        & \GP & 0.4765 & 0.5413 & 0.5872 & 0.3920 & 0.4142 & 0.4271\\
        & \IT & 0.0179 & 0.0308 & 0.0447 & 0.0121 & 0.0167 & 0.0206\\
        & $\GP$+$\IT$ & 0.4774 & 0.5453 & 0.5963 & 0.3929 & 0.4163 & 0.4304\\
        & $\IT$+$\IC$ & XXX & XXX & XXX & XXX & XXX & XXX\\
        & \method & 0.4773 & 0.5461 & 0.5957 & 0.3925 & 0.4162 & 0.4299\\
        %\cmidrule(l){2-6}
        %& imprv     & 0.1\% & 0.2\% & -0.1\% & 0.1\% \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
        \begin{footnotesize}
        \item
        \method is identical to $\GP$+$\IT$+$\IC$. 
          The best performance in each dataset is \textbf{bold}.
          The second best performance is \underline{underline}.
          %\xia{modify this table as we discussed... for sTMall under recall@10, bold 0.1226 for EMLR and underline 
          %the two 0.1226 for MLP+GP and RNN+GP, and calculate improve accordingly... }
          \par
        \end{footnotesize}
      \end{tablenotes}
  \end{threeparttable}
\end{table}


==> legend.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,720.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3206,547){\makebox(0,0)[r]{\strut{}\scriptsize{$\IT$+$\ST$}}}%
      \csname LTb\endcsname%%
      \put(4166,547){\mak    \gplbacktext
    \put(0,0){\includegraphics{legendPDF}}%
    \gplfronttext
  \end{picture}%
\endgroup
}%
    \gplfronttext
  \end{picture}%
\endgroup

